Efficient Defense Against Model Stealing Attacks on Convolutional Neural Networks

Model stealing attacks have become a serious concern for deep learning models, where an attacker can steal a trained model by querying its black-box API. This can lead to intellectual property theft and other security and privacy risks. The current state-of-the-art defenses against model stealing attacks suggest adding perturbations to the prediction probabilities. However, they suffer from heavy computations and make impracticable assumptions about the adversary. They often require the training of auxiliary models. This can be time-consuming and resource-intensive which hinders the deployment of these defenses in real-world applications. In this paper, we propose a simple yet effective and efficient defense alternative. We introduce a heuristic approach to perturb the output probabilities. The proposed defense can be easily integrated into models without additional training. We show that our defense is effective in defending against three state-of-the-art stealing attacks. We evaluate our approach on large and quantized (i.e., compressed) Convolutional Neural Networks (CNNs) trained on several vision datasets. Our technique outperforms the state-of-the-art defenses with a $\times37$ faster inference latency without requiring any additional model and with a low impact on the model's performance. We validate that our defense is also effective for quantized CNNs targeting edge devices.

==> src/ML.tex <==

% \subsection{Machine learning and neural networks}

%\textcolor{red}{TODO : remove the ML section and talk faster about DL}

% \textit{A machine learning} algorithm
% is an algorithm that can learn from data to perform a task. The data includes examples with quantitatively measured features \cite{Goodfellow-et-al-2016}. 
% An example is typically represented as a vector 
% $ \boldsymbol x \in \mathcal{R}^n$ 
% where each entry of the vector $x_i$ is another feature.
% \ac{ML} algorithms can be broadly categorized as supervised and unsupervised:


% % TODO : Supervised and unsupervised learning ??
% \begin{itemize}

% \item supervised learning algorithms involve working on annotated datasets which means every example $\boldsymbol x$ in the dataset is associated with a  provided label $\boldsymbol y$. The algorithm learns to predict $\boldsymbol y$ from $\boldsymbol x$ by estimating $p(\boldsymbol y|\boldsymbol x)$~\cite{Goodfellow-et-al-2016}, and;
% \item unsupervised learning algorithms experience an unlabeled dataset containing a collection of examples, and try to learn interesting properties about the dataset's structure~\cite{Goodfellow-et-al-2016}. The algorithm wants to learn implicitly or explicitly a probability distribution that generated the data $p(\boldsymbol x)$.

% \end{itemize}
% Other \ac{ML} algorithms do not work on just fixed data, such as reinforcement learning algorithms where the learning system interacts with a dynamic environment in which it must perform a certain goal. The system is provided with a feedback loop in terms of rewards as it takes actions in the environment, and through experience the agent learns a policy that maximizes that reward\cite{Russell2003}.
% \todo{ Semi-supervised and self-supervised learning, GANs...?}


% \begin{figure}[tbp]
% \centering
% \includegraphics[width=0.49\textwidth]{figs/neural_net.pdf}
% \caption{An illustration of a neural network with multiple layers. The input values are fed to the first layer and propagated to the following layers multiplied by weights. For each layer, the nodes output the results of an activation function to the sum of their entries. The last layer outputs probabilities for each class at the corresponding node.}
% \label{fig:neural net}
% \end{figure}
\subsection{\acf{DL}}
\ac{DL} is a set of \ac{ML} techniques that are based on \ac{ANN} 
\cite{Goodfellow-et-al-2016}. 
A \ac{NN} has $L$ layers representing the model's depth. Each layer is characterized by a width and a number of nodes called neurons. 
Each neuron performs an activation function %$g(\boldsymbol z)$ 
to the weighted sum of the output values of the previous layer's neurons. %: $\boldsymbol z= \boldsymbol W^T\boldsymbol h+\boldsymbol b$. 
The training process aims to obtain a meaningful set of weights. During the training process, parameter optimization approaches such as stochastic gradient descent (SGD) are used to minimize a certain loss function~\cite{Goodfellow-et-al-2016}.

\subsection{\acf{CNNs}}
\ac{CNNs} are a special type of \ac{NN}s that are often used in  image classification tasks. In \textit{\ac{CNNs}}, at least one of the layers should perform a mathematical convolution operation followed by a non-linear activation \cite{Krizhevsky2017}.

\kacem{TODO: write about the sota CNNs such: ResNet, VGG..}




% \rewrite{\textit{Deep learning} is a subset of \ac{ML} involving techniques based on \ac{ANN} \cite{Goodfellow-et-al-2016}.  An example of a deep learning model is a feed-forward deep network, or a \ac{MLP}, which is a mathematical function defined as $\boldsymbol y = F(\boldsymbol x)$  mapping input vectors  $\boldsymbol x \in \mathcal{R}^n$  to output  values  $\boldsymbol y \in \mathcal{R}^m$.  A \ac{NN} has $L$ layers characterizing the model's depth where each layer has a width and is characterized with a number of nodes called neurons. 
% Fig~\ref{fig:neural net} illustrates an example architecture where the neurons connect the layers together through weights $\boldsymbol W$. 
% % Each neuron perform an activation function $g(\boldsymbol z)$ to the weighted sum of the output values of the previous layer's neurons: $\boldsymbol z= \boldsymbol W^T\boldsymbol h+\boldsymbol b$.
% % To obtain a meaningful set of weights, a training process is performed and the parameters are optimized via approaches such as stochastic gradient descent (SGD) in order to minimize a certain loss function~\cite{Goodfellow-et-al-2016}.}




% \rewrite{\textit{\ac{CNNs}}
% are a particular type of feed-forward \ac{NN}s, that are mostly suitable for image classification tasks, with the requirement that at least one of the layers performs a mathematical operation called convolution operation followed by a non-linear activation. 
% After enough training, \ac{CNNs} are able to learn filters and characteristics relevant to the task \cite{Krizhevsky2017}.
% }
\subsection{\ac{CNNs} Quantization}
It is a technique used to reduce the memory footprint and computation cost of a \ac{CNN} model by representing its weights and activations using lower precision data types. 
In other words, quantizing the weights involves reducing the number of bits used to represent the parameters, typically from the standard 32-bit floating-point representation to 8-bit or even lower precision.
relies on quantizing the weights which means reducing the number of bits required to represent a parameter \cite{vanhoucke2011improving,han2015deep}. 
In some cases, we can even have  a 1-bit representation, i.e., a network with binary weights \cite{courbariaux2015binaryconnect}. Quantization enables performance gains (less memory usage and faster latency) at the expense of accuracy. 
In this paper, we consider two of the most used quantization techniques for \ac{CNNs}: \ac{PTQ} and \ac{QAT}.
% ~\cite{krishnamoorthi_pytorch_quantization}:
% https://pytorch.org/blog/introduction-to-quantization-on-pytorch/
    \ac{PTQ} finds the quantization parameters without retraining the model. It computes the resulting distributions of the different activation functions after feeding some batches of data to the trained model, in order to determine the specific quantization of each activation at inference time. Then the model is quantized based on the calibration results. This technique is fast and simple, however the quantized model may have a lower accuracy than the original one~\cite{survey_q}. 
    % https://leimao.github.io/blog/PyTorch-Static-Quantization/
   During \ac{QAT}, float parameter values are rounded to mimic int8 values, so the weight adjustments are made while being \textit{aware} that the model will be quantized. The calibration is performed while re-training the model. This technique often results in quantized models with higher accuracy than with \ac{PTQ}~\cite{survey_q}.
    % https://leimao.github.io/blog/PyTorch-Quantization-Aware-Training/









==> src/accelerator.tex <==
A neural network accelerator is a processor that is customized and optimized specifically to perform neural network operations more efficiently than general-purpose processors 
\cite{Werbos2004-NN-accelerator}. 

For domain specific applications based on DNNs and CNNs, in contrast to central processing units (CPUs) and graphics processing units (GPUs), the custom architecture of neural network accelerators enabled them to achieve a great success in both cloud and edge scenarios offering superior performance and better energy efficiency 
\cite{Chen2020-accelerator-survey}.




==> src/compression.tex <==
% \subsection{Model Compression}
% State-of-the-art \ac{DNNs} are more and more computationally expensive and requiring an intensive memory, which at some cases hinder their deployment in embedded devices and FPGAs. Therefore, during the past years researchers proposed to compress \ac{DNNs} without significantly affecting their performance to benefit from the \ac{DL} technology in several applications such as robotics and autonomous vehicles.

Proposed techniques in the state-of-the-art could be categorized into four categories: parameter pruning and quantization, low-rank factorization, transferred/compact convolutional filters, and knowledge distillation \cite{cheng2017survey}.

% \begin{itemize}
%     \item 
% Parameter pruning and quantization techniques relies on reducing redundant  and non-informative parameters. 
% Some works explore the redundancy among neurons and parameters, then proposed techniques to remove redundant ones \cite{srinivas2015data, han2015learning }. 
Parameter quantization rely on quantizing the weights which could be described as reducing the number of bits required to represent a parameter \cite{vanhoucke2011improving, han2015deep} and in some cases even a 1-bit representation, i.e., a network with binary weights \cite{courbariaux2015binaryconnect, courbariaux2016binarized}. These techniques support both training from scratch and pre-trained models.
    
    % Useless
    % \item Low-rank factorization techniques are based on using tensor/matrix decomposition to estimate informative parameters \cite{cheng2017survey}. These techniques focuse on reducing computations of convolutions as well as fully connected layers \cite{swaminathan2020sparse}. For example, a convolution filter could be approximated by a linear combination of a smaller basis filters which could be decomposed into a sequence of horizontal and vertical filters \cite{jaderberg2014speeding}. These techniques support both training from scratch and pre-trained models.
    
    % \item Transferred/compact convolutional filters methods design special structural convolutional filters to reduce the parameter space and save storage/computation \cite{cheng2017survey}. The intuition behind it is that transforming an input and then passing it to the network is equivalent to mapping the input through the network then transforming the representation\cite{cohen2016group}. For example, as shown by W. Shanget al. \cite{shang2016understanding} \ac{CNNs} learned redundant filters extracting positive and negative phase information of input signal, so they proposed a negative transformation and kept a basis convolution filter allowing them to achieve x2 compression rate. However, these techniques can only be applied to train from scratch models.
    
    
    % \item Knowledge distillation refers to methods used to distill the knowledge from a large network to a smaller one \cite{hinton2015distilling}. The compact network could be obtained by training it on synthetic data that were labeled the large complex model.  Researchers adopt different techniques to select this data or generate it, for example, to train a student network from a teacher network Hinton et al. \cite{hinton2015distilling} used a combination of data labeled by the teacher network and true labeled data. Knowledge distillation only support training a model from scratch.
% \end{itemize}

==> src/defenses.tex <==

% TODO PARAPHRASE
For each query, in order to find the right perturbation, they try to solve an optimization problem where they simulate the attacker by another network and try to add the perturbation that maximizes the error of the simulated model \cite{Orekondy2019poisoning, mazeika2022steer}.

\rewrite{Model extraction attacks have several drawbacks on \ac{ML} security and privacy, therefore, researchers propose different techniques to defend against them and mitigate their risk. 
Some techniques suggest watermarking the model to help claim it when stolen \cite{szyller2019dawn, jia2020entangled}, for example by changing the output probabilities for a small subset of queries (e.g., $\leq 0.5\%$) from API clients which allows model owners to reliably demonstrate ownership.
Other defenses can be broadly categorized into two main categories: \emph{proactive} and \emph{reactive} techniques. 
The former includes techniques to reduce efficiency of an extraction attack such as changing the prediction probabilities \cite{lee2018defending,kariyappa2020defending, Orekondy2019poisoning}. 
But, they may sometimes degrade the model accuracy and result in inference delays and an increase in computational costs.
Reactive defenses are based on the detection of extraction attacks when they are happening which enables the victim to take action immediately. 
These techniques continually observe the API query and response streams of users in order to either train a substitute model to assess the knowledge gained by the adversaries~\cite{Kesarwani2018},
or analyse the distribution of successive users queries to identify a deviation from a normal (Gaussian) distribution~\cite{Juuti2019} or a large number of OOD queries~\cite{kariyappa2020defending}.
However, these defenses do not detect all the attacks and they often consume more computational power.}

% Szyller et al. \cite{szyller2019dawn} presents \emph{DAWN} a dynamic adversarial watermarking technique of \ac{NN}s. It is based on dynamically changing the output probabilities for a small subset of queries (e.g., $\leq 0.5\%$) from API clients which allows model owners to reliably demonstrate ownership. 
% Jia et al. \cite{jia2020entangled} propose to entangle the watermarks in the model. They encourage the model to learn common features for classifying data from the task distribution as well as data encoding watermarks.

%Concerning the detection techniques, Kesarwani et al. \cite{Kesarwani2018} propose to add a model extraction monitor that continually observe the API query and response streams of users in \ac{MLaaS} paradigm. 
%They use substitute decision tree models to adapatively assess the knowledge gained by both individual and colluding adversaries, then they raise a warning whenever an extraction is detected. However, since their technique requires training a substitute model based on users queries, this solution consumes more computational power than simply deploying the model to be used as a service. 
%Juuti et al. \cite{Juuti2019} propose another approach that does not require more computational power, instead, it analyses the distribution of successive users queries and tries to identify a deviation from a normal (Gaussian) distribution. However, this technique does not detect all the attacks.

%Lee et al. \cite{lee2018defending} present a defense that aims to degrade the stolen model accuracy or require more queries for the extraction. It is based on limiting the information of the prediction probabilities of the model and misleading the adversary. They leverage the last layer in a neural network, that outputs the prediction probabilities of each class, and change its activation function to \emph{reverse sigmoid}. In that way their approach adds smart noise in the output probability that maintains the output class label of the model which forces the adversary to discard the probability and use the label only. 

%Kariyappa et al. \cite{kariyappa2020defending} propose a defense with \emph{adaptive misinformation} which defends only when it detects an attack. Their detection is based on analyzing the queries of existing model stealing attacks and observing that these attacks produce a large number of out of distribution queries. So, they leverage this observation to build their detector that flags "suspicious" inputs and serve them with incorrect predictions from an auxiliary "misinformation model". However, their technique may degrade the model accuracy on false positives.

%Orekondy et al. \cite{Orekondy2019poisoning} propose \emph{prediction poisoning}, a technique that perturbs the probabilities which is based on maximizing angular deviation. They add targeted noise to the posterior probabilities with an objective of poisoning the adversary's gradient signal. Their approach results in an adversarial gradient signal that maximally deviates from the original signal. However, this technique requires a lot of gradient calculations, which results in inference delays and an increase in computational costs.
%Zheng et al. \cite{zheng2020protecting} propose to use differential privacy to perturb the output. They add a boundary differential privacy layer that obfuscates the output probabilities of the queries. 



% \subsubsection{Discussion} 
% Defending against extraction attacks is mandatory to mitigate their risk. The discussed defense methods in the literature share a common denominator, they only consider models that were trained under default and natural training circumstances. 
% The impact of adversarial robustness techniques on extraction defense solutions has not been evaluated. 
% Furthermore, current state-of-the-art defense strategies still have some limitations, thus, improving them and proposing other ones could be a future research direction. 



==> src/ethical-statement.tex <==
\section{Ethical Statement}
% Ethics is one of the most important topics to emerge in machine learning and data mining. We ask you to think about the ethical implications of your submission such as, e.g., related to the collection and processing of personal data, the inference of personal information, or the potential use of your work for policing or the military. which will be taken into consideration by the reviewers. As part of your submission, you are asked to include an ethical statement up to one page in length that discusses any ethical implications of your work.

The protection of intellectual property and the privacy of sensitive data is paramount in machine learning, especially in the case of Convolutional Neural Networks (CNNs) used in sensitive applications. Our proposed defense mechanism against model stealing attacks on CNNs aims to safeguard such intellectual property and ensure that privacy is maintained. We believe that our work promotes the ethical and responsible use of machine learning algorithms, thereby preventing potential misuse or harm to individuals or organizations. We hope that our research contributes to the development of ethical standards in the field of machine learning and encourages responsible innovation.
In our paper, we do not collect or process any personal data and there is no potential for inference of personal information. Furthermore, our work does not have any potential use for policing or military purposes. As such, we believe that our work does not pose any ethical risks. 

==> src/extra.tex <==
\newpage





%-------- 





% -------------------



\begin{figure*}[tb]
\centering
\includegraphics[width=0.75\textwidth]{figs/dist.pdf}
\caption{\kacem{ this figure shows the distribution deviation caused by the defense, maybe top-1 is enough instead of all top-4} Distribution for the predictions of top 4 classes in GTSRB using each defense technique ... \kacem{todo: correct the legend with the real name of each defense, also change the colors so it matches other figures.}
}
\label{fig:defenses-dist}
\end{figure*}





% --------






% \kacem{add a table to describe CNN architectures + quantized models}









% \begin{table}[htbp]
% \caption{Table Template Type Styles}
% \begin{center}
% \begin{tabular}{|c|c|c|c|}
% \hline
% \textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
% \cline{2-4} 
% \textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
% \hline
% copy& More table copy$^{\mathrm{a}}$& &  \\
% \hline
% \multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
% \end{tabular}
% \label{tab1}
% \end{center}
% \end{table}




==> src/methodology-old-text.tex <==


Contrary to state-of-the-art defenses \emph{GRAD$^2$}~\cite{mazeika2022steer} and \emph{MAD}~\cite{Orekondy2019poisoning} that use computationally expensive defenses,
we propose a heuristic approach to find the perturbed predictions. We revisit previous defenses that have small inference times, i.e., \ac{RS} and \ac{AM} (Table~\ref{tab:compare}) and we propose a better alternative to overcome their limitations such as high perturbation levels or requiring an auxiliary model.
% \mouna{so for RS and AM, the limitation is not the inference time, it is just the computationally expensive thing ? maybe rewrite what limitations you want to overcome}
% in Section~\ref{sec:approach}. 
% In the rest of this section, we explain in detail these defenses to better introduce our approach.

\subsubsection{\acf{RS} \cite{lee2018defending}} 
\ac{RS} is a perturbation technique that relies on an add-on layer that aims to perturb the predictions and increase its divergence from the original posteriors.
It assumes that the attacker has perfectly stolen the victim model:
$F_A(x;\theta)=F_V(x;\theta)$.
Instead of estimating the loss for each input using a surrogate model, they use the victim's loss $L(y,F_{V}(x;\theta))$ to solve the problem. 
We find their assumption practical and we build on it later  to develop a better defense alternative. 
\ac{RS} uses a reverse sigmoid function $S^{-1}(y)=\log(y/(1-y))$ on the predictions $y$ in order to retrieve the initial logits (i.e., the obtained vectors from the last layer). Then it selects a perturbation $z=\gamma S^{-1}(y)$, where $\gamma$ is a dataset-specific constant proposed by the authors in order to have more control over the defense's convergence. After that, a sigmoid function is applied on $z$: $S(z)=1/(1+e^{-z})$. Finally, the heuristically obtained perturbation $r$ is:
\begin{equation}
    \label{eq:reverse-sigmoid}
     r(y) = S ( z) - 1/2  = S ( \gamma S^{-1}(y)) - 1/2  
\end{equation}
The model's final prediction outputs are obtained through substituting $r$ in Eq.~(\ref{eq:defense}), setting $a$ to $1$ and $b$ to a parameter  $-\beta$ that controls the noise magnitude. 
Thus, Eq.~(\ref{eq:defense}) becomes:
\begin{equation} 
\label{eq:rs}
     y'  = N( F_{V}(x ; \theta) - \beta  \cdot (S ( \gamma S^{-1}(y)) - 1/2) ) \\
\end{equation}
This technique maintains the defender's accuracy in most cases, without being computationally expensive. However, its limitation is that it uses a high perturbation, increasing the $\ell1$ distance between the clean and perturbed predictions. 
% \mouna{so, RS is fast, and not computationally expensive, its problem is just the model's transparency?, maybe you need to mention this in the introduction, that your contribution 1) reduces time, 2)not expensive and 3) improves transparency ? Also, I think a table with ticks would be great (look whiteboard) }

\subsubsection{\acf{AM} \cite{kariyappa2020defending}} 
\ac{AM} relies on perturbing only the predictions with low probabilities. 
It assumes that the queries with low probabilities are coming from an attacker, therefore the authors propose to inject a high noise into their model's output. 
% We put this in the approach and we cite them
Their technique is obtained by substituting in 
Eq.~(\ref{eq:defense}) the parameters $a\leftarrow (1-\alpha)$ and $b\leftarrow\alpha$. They define $\alpha$ as the detector function to low probability values as:
\begin{equation}
\alpha = S (\nu \cdot( y_{max} - \tau ))  \hspace{0.2cm} ;  \hspace{0.2cm} \nu=1000 \label{eq:detector}
\end{equation}
where $\tau$ is a threshold that pushes $\alpha$ towards $1$ when $y_{max} > \tau$ and towards $0$ otherwise. It is used as a switch between clean posteriors $F_{V}(x;\theta)$ and perturbed ones $r(y)$. 
To find the perturbation, they leverage another previously trained model, called \textit{misinformation model} $F_{M}(x;\theta)$. The latter is trained on the same data as the victim but in a way that maximizes the loss $ L(y,F_{V}(x;\theta))$. 
Thus, Eq.~(\ref{eq:defense}) becomes:

\begin{equation}
\label{eq:am}
     y' = N( (1-\alpha) \cdot  F_{V}(x ; \theta) +  \alpha \cdot   F_{M}(x ; \theta) ) 
\end{equation}
Their approach is effective in defending against \emph{knowledge-limited} adversaries that use \ac{OOD} queries. 
Nevertheless, it has an increased inference delay and requires an additional CNN which is the misinformation model. 
Furthermore, this technique is sensitive to false positives which deteriorates the model's performance when the queries are detected as \ac{OOD}.
% \kacem{Mention the problem with false positives too}


\subsection{Approach}
\label{sec:approach}
Our main objective is to design a defense with a low computational complexity that does not slow down the model's inference while maintaining a low perturbation. 
In contrast to the state-of-the-art defenses GRAD$^{2}$~\cite{mazeika2022steer} and MAD~\cite{Orekondy2019poisoning}, our technique does not rely on auxiliary models. 
We propose a new heuristic alternative to defend against model stealing attacks that could be applied in both large \ac{CNNs} and Quantized \ac{CNNs} for edge device implementations. 
Our technique called \acf{DCP} is inspired by both \ac{RS} and \ac{AM}. 

A strong defense that degrades the adversary's attack, aims to maximize the adversary's loss Eq.~(\ref{eq:loss_adv}).
To avoid estimating the adversary's loss through other models, 
% Instead of estimating the loss for each input using a surrogate model, they use the victim's loss $L(y,F_{V}(x;\theta))$ to solve the problem.
similar to \ac{RS} we assume that the attacker has perfectly duplicated the victim model. Thus, we use the victim's predictions as starting point to compute the perturbations.
Our strategy in injecting the noise is to decrease the uncertain probabilities. 
% and to increase the certain ones. 
Our rationale is that probabilities with low values are of less importance. We assume that if a \textit{well-trained} model is uncertain about the prediction of input, it is highly probable that the model made a wrong prediction (false positive). 
Hence, modifying these probabilities will not affect the defender's accuracy $Acc(F_{V})$. 
However, if the model predicts an output with a high probability, it is more likely that it is a correct prediction (true positive). Thus, the injected noise is minimal without affecting the defender's performance. 
% possible limitation, CIFAR-100 results, the victim model has already high error, which makes it harder to steal
We make sure that, at the same time, we respect the perturbation budget constraint Eq.~(\ref{eq:l1-distance}). 


% We  propose  3 new heuristic techniques to defend against model stealing attacks: 
%\mouna{make sure to explain how "add a higher perturbation to uncertain probabilities" in each of these below}
% \subsubsection{\acf{Soft-RS}}
% this technique is based on the \ac{RS} defense. However, in order to apply our strategy, we choose to change  the activation function from \eqref{eq:reverse-sigmoid} to a softplus, defined as $\zeta(z)$, instead of a sigmoid $S(z)$, obtaining the following function:
% \begin{equation}
%       y' = N( F_{V}(x ; \theta) -  \beta \cdot ( \zeta( \gamma . S^{-1}(y)) - 1/2)
% \end{equation}
% where  $\zeta(z)=\log(1 + e^{z})$, $\beta$ is a perturbation magnitude parameter that we tune in order to find the suitable perturbation that respects the problem constraints and $\gamma$ is a dataset specific constant.

% \subsubsection{\acf{DCP}} 
% We  propose  a new heuristic technique to defend against model stealing attacks called \acf{DCP}.
% This technique is inspired by both \ac{RS} and \ac{AM}. 
In order to heuristically find which posteriors to perturb, we leverage Eq.~(\ref{eq:detector}) to control our noise. 
However, instead of using an extra model to inject the noise, we utilize
Eq.~(\ref{eq:reverse-sigmoid}) as a noise function in 
Eq.~(\ref{eq:defense}). 
In contrast to \ac{AM} that multiplies $F_{V}$ by $(1-\alpha)$ in Eq.~(\ref{eq:dcp}) to create a combination between the clean posteriors and the noise, which results in deteriorating the defender's performance in case of false positives, we set the parameter $a\leftarrow1$ and $b\leftarrow-\beta\cdot\alpha$ to finally obtain: 
%---------- equations
\begin{equation} 
\label{eq:dcp}
     y'  = N( F_{V}(x ; \theta) - \beta \cdot S (\nu \cdot( y_{max} - \tau )) \cdot (S ( \gamma S^{-1}(y)) - 1/2) ) \\
\end{equation} 

% $ \alpha = S ( y_{max} - \tau );  \tau = \beta $ and $S =  \frac{\mathrm{1} }{\mathrm{1} + e^{\nu z} } $
where $S$ and $S^{-1}$ are respectively the sigmoid and reverse sigmoid functions. We set $\tau \leftarrow \beta$ to control the perturbation magnitude.
With this setting we have  $ y' \rightarrow  F_{V}(x; \theta) $ when $ \alpha \rightarrow 0 $  and  $ y'\rightarrow  RS $ when $ \alpha \rightarrow 1$. 
% Our aim is to avoid deteriorating the defender model's performance without

% $ \alpha \rightarrow 0 , \hat{y} \rightarrow  F_{V}(x; \theta) $
% $ \alpha \rightarrow 1 , \hat{y} \rightarrow  RS $


% \subsubsection{\acf{CDCP}} This technique builds upon \ac{DCP}. Additionally, we multiply $F_{V}$ by $(1-\alpha)$ in \eqref{eq:dcp} in order to transform it to create a combination between the clean posteriors and the noise. This technique adds more control on the used fraction of the original prediction probabilities in the final perturbed posteriors. Using $\alpha$ from~\eqref{eq:detector}, we obtain:
% % \alphaS (\nu \cdot( y_{max} - \tau ))
% \begin{equation}
%      y' = N( (1-\alpha)  F_{V}(x ; \theta) +  \beta \cdot \alpha \cdot  (S ( \gamma S^{-1}(y)) - 1/2) )
% \end{equation}

% With this setting we have  $ y' \rightarrow  F_{V}(x; \theta) $ when $ \alpha \rightarrow 0 $  and  $ y'\rightarrow  r $ when $ \alpha \rightarrow 1$.



%----------------


==> src/sota.tex <==

% part for literature review



% Useless section
% \subsection{Neural network accelerator}
% \label{sec:accelerator}
% \input{src/accelerator}

% Useless section, quantization part is inserted in ML section
% \subsection{Model compression}
% \label{sec:compression}
% \input{src/compression}

\subsection{Model stealing attacks (model extraction attacks)} 
\label{sec:background-sota}
\input{src/related work}

\subsection{Defenses against model stealing attacks}
\label{sec:defenses}
\input{src/defenses}




\subsection{Positioning with the state-of-the-art} 
% Explain here what is original in this paper
% The extraction attacks raise risks on the intellectual property of \ac{ML} models and it may facilitate other adversarial attacks. 
% Stealing attacks are diverse and were proven to be successful in many cases, yet they were only demonstrated on unaltered and standard sate-of-the-art models that were trained under natural training circumstances. 
% They still do not consider security-imposed scenarios that modify the model's architecture or its behavior for instance towards adversarial examples. 
% Adversarial training impacts the prediction probabilities that could be leveraged by malicious users to perform other attacks through observing the model's response to their queries.
% Particularly, adversarially robust models were proven to be more vulnerable to membership inference attacks due to their wider generalization compared to natural models which raises concerns about the training data privacy~\cite{song2019privacy}. 
% Extraction attacks rely on the predictions probabilities of the victim model to the adversary's queries and have not yet been evaluated on adversarially robust models, hence, the extraction robustness of the latter is still an open research problem.
% It is unknown if we alter the models through adversarial training, we increase or not their vulnerability to extraction.
% % Our paper seek to lessen this research gap with a new approach and significant empirical study. 
% In order to answer to this question, we propose a new methodology and a significant empirical study.




